Exact Spectral Norm Regularization for Neural Networks

We pursue a line of research that seeks to regularize the spectral norm of the Jacobian of the input-output mapping for deep neural networks. While previous work rely on upper bounding techniques, we provide a scheme that targets the exact spectral norm. We showcase that our algorithm achieves an improved generalization performance compared to previous spectral regularization techniques while simultaneously maintaining a strong safeguard against natural and adversarial noise. Moreover, we further explore some previous reasoning concerning the strong adversarial protection that Jacobian regularization provides and show that it can be misleading.

==> hist_plot.tex <==
\begin{figure}[h]
\centering


\begin{tikzpicture} [transform shape, scale = 1.5]

\tikzstyle{arrow} = [thick,->,>=stealth]

\newcommand\imgWidth{0.2}

\node[inner sep=0pt] (expandedImg) at (0, 0)
    {\includegraphics[width=0.32\textwidth]{fw_vs_yo_leg_inside.pdf}};
    
% \node[inner sep=0pt] (expandedImg) at (-4.7, 0)
%     {\includegraphics[width=0.34\textwidth]{figures/noise_robust.pdf}};
    
% \node[scale = 0.6] at (0.1, -1.7) {Iterations};
% \node[scale = 0.6] at (-4.85, -1.7) {$\sigma$};

\end{tikzpicture}

\caption{The difference in spectral norm for two networks regularized with the Spectral and Spectral-Bound methods respectively. The histograms are constructed from 1000 randomly chosen train and validation points on KMNIST and FashionMNIST and for each point the spectral norm of the associated $W_R$ is calculated. It can be seen that the Spectral method results in lower spectral norms in general.}
\label{fig:hist}
\end{figure}
















